StealthRank: LLM Ranking Manipulation via Stealthy Prompt Optimization

The integration of large language models (LLMs) into information retrieval systems introduces new attack surfaces, particularly for adversarial ranking manipulations. We present $\textbf{StealthRank}$, a novel adversarial attack method that manipulates LLM-driven ranking systems while maintaining textual fluency and stealth. Unlike existing methods that often introduce detectable anomalies, StealthRank employs an energy-based optimization framework combined with Langevin dynamics to generate StealthRank Prompts (SRPs)-adversarial text sequences embedded within item or document descriptions that subtly yet effectively influence LLM ranking mechanisms. We evaluate StealthRank across multiple LLMs, demonstrating its ability to covertly boost the ranking of target items while avoiding explicit manipulation traces. Our results show that StealthRank consistently outperforms state-of-the-art adversarial ranking baselines in both effectiveness and stealth, highlighting critical vulnerabilities in LLM-driven ranking systems. Our code is publicly available at $\href{https://github.com/Tangyiming205069/controllable-seo}{here}$.

==> tables/ablation.tex <==
% \begin{table}[h]
%     \centering
%     \resizebox{\columnwidth}{!}{ % 让表格自动适应单栏
%     \begin{tabular}{c c ccc}
%         \toprule
%         \multicolumn{5}{c}{\textbf{Coffee Machine}} \\ % 合并5列，作为表格第一行
%         \midrule
%         \textbf{Model} & \textbf{Method} & \textbf{Rank $\downarrow$} & \textbf{Perplexity $\downarrow$} & \textbf{Bad Word Rate $\downarrow$} \\
%         \midrule
%         \multirow{4}{*}{\textbf{Llama-3.1-8b}} & Ours & $1.2 \pm 0.42$ & $71.91 \pm 21.38$ & $0.3167 \pm 0.0252$ \\
%         & Target & $1.6 \pm 1.26$ & $60.37 \pm 19.19$ & $0.6157 \pm 0.0305$ \\
%         & Ngram & $1.8 \pm 0.92$ & $115.19 \pm 51.07$ & \boldmath$0.0909 \pm 0.0250$ \\
%         & Fluency & \boldmath$1.1 \pm 0.32$ & \boldmath$59.27 \pm 17.34$ & $0.8055 \pm 0.0231$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Ablation Results for Llama-3.1-8b}
%     \label{tab:performance_comparison}
% \end{table}

\begin{comment}
\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c c ccc}
        \toprule
        \textbf{Method} & \textbf{Rank} $\downarrow$ & \textbf{Perplexity} $\downarrow$ & \textbf{Bad Word Rate} $\downarrow$ \\
        \midrule
        \textbf{Ours (Full)} 
            & $1.2 \pm 0.42$ 
            & $71.91 \pm 21.38$ 
            & $0.3167 \pm 0.0252$ \\
        \textbf{Rank Only} 
            & $1.6 \pm 1.26$ 
            & $60.37 \pm 19.19$ 
            & $0.6157 \pm 0.0305$ \\
        \textbf{High N-gram} 
            & $1.8 \pm 0.92$ 
            & $115.19 \pm 51.07$ 
            & \textbf{0.0909} $\pm$ 0.0250 \\
        \textbf{High Fluency} 
            & \textbf{1.1} $\pm$ 0.32 
            & \textbf{59.27} $\pm$ 17.34 
            & $0.8055 \pm 0.0231$ \\
        \bottomrule
    \end{tabular}
    }
    \vskip-2mm \caption{Ablation on Llama-3.1-8B (Coffee Machine). ``Bad Word Rate'' reflects restricted ranking terms.} \vspace{-6mm} 
    \label{tab:performance_comparison}
\end{table}
\end{comment}

\begin{comment}
    \begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c c ccc}
        \toprule
        \textbf{Method} & \textbf{Rank} $\downarrow$ & \textbf{Perplexity} $\downarrow$ & \textbf{Bad Word Rate} $\downarrow$ \\
        \midrule
        \textbf{Ours (Full)} 
            & $1.2 \pm 0.42$ 
            & $71.91 \pm 21.38$ 
            & $0.3343 \pm 0.0255$ \\
        \textbf{Rank Only} 
            & $1.6 \pm 1.26$ 
            & $60.37 \pm 19.19$ 
            & $0.6157 \pm 0.0305$ \\
        \textbf{High N-gram} 
            & $1.8 \pm 0.92$ 
            & $115.19 \pm 51.07$ 
            & \textbf{0.1439} $\pm$ 0.0306 \\
        \textbf{High Fluency} 
            & \textbf{1.1} $\pm$ 0.32 
            & \textbf{59.27} $\pm$ 17.34 
            & $0.8430 \pm 0.0213$ \\
        \bottomrule
    \end{tabular}
    }
    \vskip-2mm \caption{Ablation on Llama-3.1-8B (Coffee Machine). ``Bad Word Rate'' reflects restricted ranking terms.} \vspace{-6mm} 
    \label{tab:performance_comparison}
\end{table}
\end{comment}

% \begin{table}[!ht]
%     \centering
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{c c ccc}
%         \toprule
%         \textbf{Method} & \textbf{Rank} $\downarrow$ & \textbf{Perplexity} $\downarrow$ & \makecell{\textbf{Bad Word Ratio} \\ \textbf{(After 1000)} $\downarrow$} \\
%         \midrule
%         \textbf{Ours (Full)} 
%             & $1.2 \pm 0.42$ 
%             & $71.91 \pm 21.38$ 
%             & \textbf{0.0645} $\pm$ 0.0133 \\
%         \textbf{Rank Only} 
%             & $1.6 \pm 1.26$ 
%             & $60.37 \pm 19.19$ 
%             & $0.6157 \pm 0.0305$ \\
%         \textbf{High N-gram} 
%             & $1.8 \pm 0.92$ 
%             & $115.19 \pm 51.07$ 
%             & $0.1515$ $\pm$ 0.0312 \\
%         \textbf{High Fluency} 
%             & \textbf{1.1} $\pm$ 0.32 
%             & \textbf{59.27} $\pm$ 17.34 
%             & $0.8771 \pm 0.0192$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \vskip-2mm \caption{Ablation result on Llama-3.1-8B (Coffee Machine). \textbf{Note}: ``Bad Word Rate'' here reflects the occurrence of restricted ranking terms in prompts sampled after 1000 training iterations.} 
%     \vspace{-3mm} 
%     \label{tab:performance_comparison}
% \end{table}
